Popularity Driven Data Integration

More and more, with the growing focus on large scale analytics, we are confronted with the need of integrating data from multiple sources. The problem is that these data are impossible to reuse as-is. The net result is high cost, with the further drawback that the resulting integrated data will again be hardly reusable as-is. iTelos is a general purpose methodology aiming at minimizing the effects of this process. The intuition is that data will be treated differently based on their popularity: the more a certain set of data have been reused, the more they will be reused and the less they will be changed across reuses, thus decreasing the overall data preprocessing costs, while increasing backward compatibility and future sharing

==> sec_02_soa.tex <==
\section{DI strategies} \label{sec2_soa}

% Data availability increase the need for:

% integrate data in many different domains, defining thus a general purpose demand for integration solutions. 

% such solutions have to be designed to satisfy also very specif purposes

% Specific purpose application
% brings to over fitted structure where organize and maintain integrated data.
% P1 -> no extensible in time
% P2 -> no reusability , negative loop


%The amount of data and relative information, nowadays available, increases the need of integration solutions able to exploit heterogeneous data through single applications/services. We detail in this section, the problem of defining a general purpose DI strategy, able to produce reusable resources. Then the analysis of existing DI strategy is reported, explaining which are the limits of such strategies in solving the problem stated.

%\subsection{The problem}

%The context in which data integration is requested can vary a lot, from business enterprise contexts, collecting data from big data sources like data warehouse and data lakes [CITATIONS], to smaller context such as the management of personal information within your PC. It clearly appears how the purpose for which the integration outcome is produced, changes consequently from one context to one another. Not only the context of data retrieval, but also the exploitation of the integration outcome, increases the number of possible purposes to be considered. In fact, DI integration can be exploited for many different objectives, such as integration of existing data, generation of information structures (databases, KGs) later populated with incoming data, statistical analysis and many other applications in several domains of interest. Such wide range of possible DI purposes, implies difficulties in the definition of standards general purpose methodologies and frameworks.


% increased data availability, and accessibility, leads also to the exploitation of DI for very specific purposes. A perfect example of this scenario are the Personal Management Information system (PIMs)[CITATIONS], used by single persons to integrate their own information. Clearly the application of such systems can have very specific purposes referred to any single aspects of the person's life (i.e. integrate all the information about a single person's vacation, such as photos, videos, notes, GPS traces, and others). The design of such kind of specif purpose services, brings often to model data structures over fitted on data, thus hardly extensible and reusable out of the purpose of their creation. The missing of reusable resources (like data and data schemas) increases, consequently, the effort in data collection and information modelling activities, thus often falling back to the generation of new over fitted resources. It is a negative loop which consistently reinforces itself, producing specif purpose resources, which in turn have to be remodeled from scratch to satisfy new requirements, or extending the original ones. Within the existing data integration strategies, we identified a lack of methodologies and frameworks which can be applied in any possible domain of interest. Moreover, the results obtained by the existing DI solutions, are not reusable enough in different domains (or integration purposes). Due to that the negative reusability loop is not yet broken, thus keeping higher the effort required within the integration process. In support of this claim, we reported, in the next sub section, the analysis of the existing DI strategies, and their limitations with respects the problems expressed above. 



Major improvements in DI have been produced thanks to the studies on Semantic Web. Due to that the ontology-based DI (OBDI) approach \cite{2001-obdi} is now considered for many applications. The key objective of OBDI techniques is to produce a unique representation of the information carried by data provided by different sources. OBDI approach aims to share the data models used by each source with the consequent objective to build a global data model (global ontology) able to provide a unified representation of the data. The existing OBDI strategies can be collected within two different categories, called virtualization and materialization.

\textit{Virtualization strategies} aim to provide a unique view over multiple data sources, without extraction and transformation of their data. That is why they are also known as Ontology Based Data Access (OBDA). Virtualization strategies build a unique view of data, on which the queries are posed, allowing software applications to exploit the integration result. The queries posed to the global view, are then translated into queries on single sources data models, allowing the effective information retrieval. In \cite{2017-obdi-for-mdee} Ekaputra et al. report different DI solutions which differs based on how they produce a global view over multiple data sources. The global view can be build as a single ontology modeled over the different data sources model. Such approach unifies the data sources information but is typically hard to maintain because it is susceptible to changes in each data source. Other OBDA approaches define multiple ontologies, one for each data sources, defining then semantic mapping between them (multiple-ontology OBDI). A different approach, instead, adopts a unique vocabulary to define each single local ontology (hybrid OBDI), simplifying the ontology definition as well as the query building. A composition of the previous solutions has been produced by defining both multiple local ontologies and a single global one, then defining mappings between the local and global layer (\textit{Global-As-View} OBDI). The different OBDA approaches can be in general described by two main features. (i) They integrate the access to data sources more than the data collected within them. (ii) Leaving out the single-ontology approach having more high maintenance cost, OBDA strategies require the definition of multiple ontologies as well as the respective mappings between them. Due to the two features above, OBDA strategies are more suitable for applications which need a unified access to multiple sources than for those exploiting a single information structure, thus having a direct control over the data.


\textit{Materialization strategies} are based on ETL procedures used to extract the data to be integrated from the respective data sources. The subsequent objective is to create a single information structure able to maintain the heterogeneous data collected. Therefore providing a single object for data management and exploitation. Compared with virtualization strategies, materialization ones work directly on data extracted from the sources, building a single global ontology for the data extracted, thus reducing the effort in building multiple ontologies (and relative mappings). Nevertheless, materialization strategies have to deal with the heterogeneity of the data extracted from different sources. Such heterogeneity can be recognized on different levels within the datasets collected, at language level (in case of cross country data integration), at conceptual level (when a real word entity is represent by different properties in different datasets) and at single values level (different data format and standards adopted by different datasets). In \cite{2020-Stratified-DI} Giunchiglia et al. propose an efficient solutions which aims to handle the different levels of heterogeneity through different Knowledge Graphs (KGs). Those KGs are then composed together to build a single object able to maintain and exploit heterogeneous data. More in general the usage of KGs increased a lot within the data integration community, thanks to their exploitability in many different domain of interest, such as sustainable transportation \cite{2021-kg-for-battery}, biomedical data \cite{2021-kg-biomedical} as well as disaster management \cite{2019-KG-embedding}, and many others. DI based on KGs construction (KGC) aims to model a single knowledge representation which must be able to satisfy the integration requirements. The existing KGC-based DI frameworks and tools are defined on single domains of interest, by exploiting a fixed knowledge representation when the global schema is built. In other words, there is always a domain specific ontology, that is used on top to construct the ontology specific for the integration requirements. Some approaches have been proposed considering as base knowledge a more general ontology (allowing suitability for more domains), like \textit{Schema.org}. Adding extensions to the top level ontology, these solutions aim to represent more domain specific aspects required for the integration objective \cite{2020-kg-intro}. Nevertheless this approach produces KGs that are more specific, and less reusable in other domains, the higher is the number of extensions added to the original standard schema (i.e. Schema.org).







==> sec_07_evaluation.tex <==
\section{Alignment Evaluation} 
\label{sec7_evaluation}

\vspace{-0.1cm}
The evaluation is based on a set of metrics that are applied to CQs, ETGs, datasets, and dataset schemas, where the latter - when they are not KGs - are treated as sets of properties associated with one or more selected etypes of the ETG. These metrics are applied in the four phases of the \itelos\ process. For lack of space, below we describe only the application of three metrics to a specific phase.

Let $\alpha$ and $\beta$ be two generic \textit{element} sets, where an element can be an etype or a property. We have the following:

\vspace{0.1cm}
\noindent
 \textit{Coverage}. This metric allows to ascertain the extent to which an element set is appropriate for the purpose, and it is computed as the ratio between the intersection of $\alpha$ and $\beta$ and the whole $\alpha$. 
 \vspace{-0.2cm}
    \begin{equation}
    \label{eq1}
    Cov = (\alpha \cap \beta) / \alpha
    \end{equation}
    
\vspace{-0.1cm}
\noindent For instance, during the inception phase (\textit{Eval(a)} in Figure \ref{fig:pipeline}), \(Cov\) plays a central role in evaluating the \emph{reusability} of potential datasets (via dataset schemas) with respect to the CQs. For each dataset, a high value of \(Cov\), both applied to etypes and properties, implies that the dataset is highly appropriate for the purpose. A low value of \(Cov\) implies minimal overlap between the purpose and the dataset, the consequence being non-consideration of the dataset for reuse, and possible modification of the (underspecified) CQs. 
%Finally, after examining an appropriate number of datasets according to project requirements, we have a \emph{reusable collection of datasets}, which exhibit \emph{maximum convergence} with respect to the CQs (especially a complete or, at least, a high overlap, with respect to the common etypes and properties from CQs).
    
\vspace{0.1cm}
\noindent
\textit{Extensiveness}. This metric quantifies the proportional amount of knowledge provided by any element set (such as $\beta$), in terms of set of etypes or of sets of properties, with respect to the entire knowledge considered (here $\alpha$ and $\beta$)
 \vspace{-0.1cm}
    \begin{equation}
    \label{eq2}
    Ext = (\beta - (\alpha \cap \beta)) / ((\alpha + \beta) - (\alpha \cap \beta))
    \end{equation}
\noindent During the Modeling phase (\textit{Eval(b)} in Figure \ref{fig:pipeline}), the evaluation utilizes \(Ext\) to ensure that the ETG model maximally extends the set of CQs, which makes the model easily amenable for further evolution. To that end, a high value of \(Ext\) is evaluative of the fact that the ETG extends the scope of the CQs, by indicating a limited contribution of the CQs in generating the ETG model. On the other hand, low values of \(Ext\) are evaluative of the fact that CQs have contributed significantly towards enhancing the ETG model. 
%Furthemore, in Modeling phase  (\textit{Eval(c)} in Figure \ref{fig:pipeline}), a low value of \(Ext\) tells us that we have an ETG model which exhibits \emph{maximum convergence} with respect to the CQs.

\vspace{0.1cm}
\noindent
 \textit{Sparsity}. This metric quantifies the element-level difference between any number of similar  element sets, and is defined as the sum of the percentage of $\alpha$ not in $\beta$, and vice versa.
  \vspace{-0.2cm}
    \begin{equation}
    \label{eq3}
    Spr = ((\alpha + \beta) - 2(\alpha \cap \beta)) / ((\alpha + \beta) - (\alpha \cap \beta))
    \end{equation}
     
\vspace{-0.2cm}
\noindent 
In the knowledge alignment phase (\textit{Eval(c)} in Figure \ref{fig:pipeline}), our principal focus is to utilize \(Spr\) for ensuring the \emph{sharability} of the ETG. We incrementally enforce sharability by ensuring a required threshold of \(Spr\) between the ETG and each of the reference ontology, which indicates that the ETG contains axioms reflective of \emph{contextual knowledge}. 

\vspace{0.2cm}
\noindent
All the above metrics operate at the schema level. But they do not say anything about the results of integrating the datasets, as caused by the semantic heterogeneity existing among them. The situation is as follows. Assume that $D1$ and $D2$ are two datasets. Let us assume that, using \textit{KarmaLinker}, we analyze first $D1$ and then $D2$. Then we have the following possible situations:
\begin{itemize}
\vspace{-0.1cm}
    \item $D2$ contains an etype which is also contained by $D1$. In this case the EG is not extended; only the number of links across nodes is increased. We have two situations depending on whether an entity populates both datasets or only one. In the first case the entity will be enriched with a new set of property values with the possibility of contradictory information. In the second case, the two different sets of entities will values only for the properties  shared between $D1$ and $D2$. This case will result in an EG with a lot of missing links.
    \item $D2$ contains a new etype with respect $D1$. In this case, the EG is extended with new nodes and new links. We have again two situations depending in whether an entity populates both datasets or only one. In the first case the EG is nicely extended by attaching new links to the entities in $D1$. In the second case the two parts of the EG resulting from the import of the two datasets will be not connected.
\end{itemize}

\vspace{-0.1cm}
\noindent
The data driven metrics briefly introduced above are crucial for the evaluation of the quality of the final EG. At the moment, these characteristics of the EG have been evaluated with a set of techniques \textit{ad hoc}. A set of metrics for the evaluation of the quality of the final EG are under definition.

% During the inception phase (\textit{Eval(a)} in Figure \ref{fig:pipeline}) the evaluation covers \emph{CQs and ontologies} (for the schema level) and \emph{CQs and Datasets} (for the data level). For the schema level, a high value of \(Cov\) implies that the ontology is highly appropriate for the purpose. A low value of \(Cov\) implies minimal overlap between the purpose and the ontology, the consequence being non-consideration of the ontology for reuse, and/or possible modification of the (underspecified) CQs. On the other hand, high values of \(Ext\) is evaluative of a high degree of diversity of the knowledge in CQs, which implies that the contribution of the knowledge content of the ontology is limited towards fulfilling the purpose and thus lower on the scale of reusability, and vice versa. The evaluation for data level is similar as above parameterized over CQs and datasets with one additional metric \(Spr\) whose high value implies diversity between the datasets and the purpose, and vice versa. Further, the same metrics are also employed to compare the convergence between each ontology and each dataset collected. Finally, after requisite refinements (as required), we have a \emph{reusable collection} of ontologies and datasets, which exhibit \emph{maximum mutual convergence} with respect to the CQs (especially a complete or, at least, a high overlap, with respect to the common etypes and properties from CQs).

% During the modeling phase (\textit{Eval(b)} in Figure \ref{fig:pipeline}), the evaluation covers the following comparisons - \emph{ETG model with ontology collection} (for the schema level) and \emph{dataset schemas with ETG model} (for the data level). For the schema level, a high value of \(Cov\) with respect to each of the collected ontology implies that the ETG model is highly appropriate for the purpose. A low value of \(Cov\), on the other hand, implies minimal overlap between them, the consequence being further refinement and evolution of the ETG model. Further, high values of \(Ext\) is evaluative of a limited contribution of the knowledge content of the ETG model towards fulfilling the purpose, and and vice versa. The evaluation for the data level can lead to either of the following three scenarios. The \emph{first scenario} occurs when the comparison yields high diversity for the dataset schema with respect to the ETG model, implying high level of sparsity leading to non-consideration of the dataset. The \emph{second scenario} occurs when the comparison results in same etypes characterized by different properties, with two possible options - extension of the ETG model with new properties to fit the dataset or non-consideration of the dataset (only if there is high diversity in properties). The \emph{third scenario}, that of same etype and properties, occurs as a result of least sparsity and leads to direction consideration of the dataset. Finally, after requisite refinements (as required), we have a \emph{reusable ETG model} and a filtered set of \emph{reusable datasets}, which exhibit \emph{maximum mutual convergence} with respect to the purpose (ideally a complete overlap with the common and core etypes and properties elicited from the purpose).

% In the knowledge alignment phase (\textit{Eval(c)} in Figure \ref{fig:pipeline}), we first evaluate the \emph{sharability} of the ETG by assessing its overlap (and divergence) with respect to the selected set of reference ontologies, by employing \(Cov\) and \(Ext\). If a full overlap, by which we mean 100\% coverage and 0\% diversity parameterized over common, core and contextual etypes and properties is noticed, it is deemed for the ETG to proceed for the final data integration phase. Otherwise, it is re-channelled for iterative ETG alignment till the desired degree of coverage is attained. On the other hand, we also perform data quality assessment to evaluate the dataset cleaning outcomes, and to that end we define the following dimensions- \emph{completeness, consistent representation} and \emph{free-of-error} \cite{pipino2002data}. Completeness evaluates \emph{``the extent to which data is not missing"} \cite{pipino2002data} (such as column completeness) and thus incentivizes to improve data sparsity. The issue of consistent representation deals with whether the datasets representationally conform to the ETG (such as in mutual alignment of datatypes). The free-of-error dimension, as distinct from that of completeness, examines data correctness, i.e. the extent to which erroneous data units are present in a dataset. Another mandatory data quality dimension, especially from an ethical point of view, involves examination (and if required, refinement) of whether individual private details are obfuscated in the datasets.
%Finally, for the data integration phase (\textit{Eval(d)} in Figure \ref{fig:pipeline}), we evaluate whether the EG is suitable enough to answer the CQs. To that end, we examine the \(Cov\) and \(Ext\) of the schema level of the EG with the CQ list. A complete overlap between them would imply that the EG is fully competent to answer the CQs, whereas, in the case of an incomplete overlap, the flow moves downstream to the knowledge alignment phase for possible refinement.

